Risk-Aware Sensitive Property-Driven Resource Management in Cloud Datacenters

Organizations are increasingly moving towards the cloud computing paradigm, in which an on-demand access to a pool of shared configurable resources is provided. However, security challenges, which are particularly exacerbated by the multitenancy and virtualization features of cloud computing, present a major obstacle. In particular, sharing of resources among potentially untrusted tenants in access controlled cloud datacenters can result in increased risk of data leakage. To address such risk, we propose an efficient risk-aware sensitive property-driven virtual resource assignment mechanism for cloud datacenters. We have used two information-theoretic measures, i.e., KL-divergence and mutual information, to represent sensitive properties in the dataset. Based on the vulnerabilities of cloud architecture and the sensitive property profile, we have formulated the problem as a cost-drive optimization problem. The problem is shown to be NP-complete. Accordingly, we have proposed two heuristics and presented simulation based performance results for cloud datacenters with multiple sensitivity.

==> assignment.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proof}{Proof}[section]

Based on the aforementioned  knowledge profile associated with RBAC policy and the virtual resource vulnerability model related to the cloud \cite{almutairi2014risk}, we now formally define the sensitive property based risk-aware  assignment problem (SPRAP) as follows: 

\begin{definition}\label{def:SPRAP}
(SPRAP). Given the knowledge profile of RBAC policy generated  based on the sensitive property function $f$, and the vulnerability matrix  $\mathcal{D}$ representing the virtual resources probability of leakage \cite{almutairi2014risk},   the sensitive property based risk-aware role assignment problem (SPRAP) is to minimize the total risk of sensitive property  disclosure by assigning access control roles to the virtual resources.
\end{definition} 

Formally, the $SPRAP$ optimization problem is given as:
\begin{equation}\label{eq:cost}
\begin{split}
\textit{minimize} \ Risk &= \sum_{r_i \in R} Risk(r_i) \\
&= \sum_{r_i \in R} \max_{A \in \mathcal{P}(R)} g_i^{A}\times Threat(A,r_i) \\
& \ \ \ \ \ \times \prod_{r_j \in A,r_j \neq r_i} d_{I(r_i),I(r_j)} 
\end{split}
\end{equation}

Such that:\\
\begin{equation}
g^A_i=  |f(A)-f(r_i)|
\end{equation}

\begin{equation}
Threat(A,r_i) =
  \begin{cases}
    1 & \quad  \text{if $r_i \in A$}\\
        0 & \quad \text{Otherwise}
  \end{cases}
\end{equation}

Where: \\
$R$: the set of roles\\
$\mathcal{P}(R)$: the power set of roles excluding the empty set\\
$A$: is subset of $\mathcal{P}(R)$\\
$I$: is the assignment function where $I(r_i)=v_j$ if role $r_i$ assigned to VM $v_j$\\
$f$: is the sensitive property function \\
$g^A_i$: is the quantitative measure associated with a sensitive property leaked to role $r_i$ when it attack the set of roles $A$ \\
$d_{i,j}$: is probability of leakage between VM $v_i$ and  VM $v_j$ 

\begin{theorem}
SPRAP problem is NP-complete.
\end{theorem} 
\begin{proof}
We construct a decision  formulation of SPRAP problem as follow:\\
For a given constant $c$, is there any assignment  $I$ such that 
\begin{eqnarray*}
Risk&=&\sum_{r_i \in R} \max_{A \in \mathcal{P}(R)} g_i^{A}\times Threat(A,r_i) \\
&\times& \prod_{r_j \in A,r_j \neq r_i} d_{I(r_i),I(r_j)}  \le c
\end{eqnarray*}
First, given $c$ and $I$ we can check if the SPRAP decision problem satisfies the bound in polynomial time. Accordingly, the decision formulation of SPRAP is NP. Next, we show that decision SPRAP problem is NP-Complete by showing that  Travel Salesman problem (TSP) can be reduced to SPRAP. We formulates TSP for a given set $U$ with a distance metric $h(a,b)$ where $a,b \in U$, is there such an ordering of elements of $U$:($u_1,u_2,...,u_m$) such that $\sum_{i=1}^n h(u_i,u_{i+1})+h(u_n,u_1) \leq c$.

Let  $f$ be the sensitive property function for  RBAC policy with $n$ roles where $R= \lbrace r_1,r_2, \dots , r_n \rbrace$.  We define $f$ as follows:
\[ f(A) = \left  \{
  \begin{array}{l l}
    1 & \quad  \text{if} \ A = \lbrace r_i, r_j \rbrace\ \text{and} \ |i-j| \ mod \ n = 1\\
    0 & \quad \text{Otherwise}
\end{array} \right.\]

Let  $V = U$  and $d_{i,i} = h(a,b)$ where $v_i= a \ \text{and} \ v_j = b$ then assume the assignment of role $r_i$ to VM $v_j$ as if the salesman visits city $u_j$. Therefore, if we find an optimal order of visits in TSP, we can find the optimal assignment of $R$  to $V$ in SPRAP.
\end{proof} 


==> performance.tex <==
In this section, we introduce three metrics to compare the performance of the proposed BFH and TDH. The first two metrics are concerned with the overall disclosure risk exhibited by all roles. The third metric focuses on the disclosure risk incurred per role. The formal definitions of these metrics are presented in this subsection and the experiment results are given in the next section. 

The  disclosure risk associated with sensitive property is the main metric that needs to be minimized and is computed over all roles. This metric depends on the  sensitive property function used in the cost function. The risk  metric associated  with $Div$ property, represented  as $RISK_{Div}$, measures the risk incurred due to the reduction in the distance between the attacker p.m.f. and the global p.m.f.. In essence, $Div$ indicates how close is the attacker's p.m.f. to the global p.m.f.. The risk metric corresponding to $MI$, denoted as $RISK_{MI}$, measures the risk incurred due to the reduction in the difference between the estimated $MI$ by a role and the global $MI$. Formally, these risk metrics are given as:\\
\begin{definition}
For the cost function associated with  $RISK_{Div}$ as per definition of Equation \ref{eq:cost}., we define the measure of disclosure  $g_i^A$ as following: \\
\begin{eqnarray*}
g_i^A &= &|D(P_A(X,Y) \parallel P_G(X,Y))\\
& -&D(P_{r_i}(X,Y) \parallel P_G(X,Y)) |
\end{eqnarray*}
Where:\\\
$P_A(X,Y)$: is the joint probability mass function  calculated based on data accessed by  the set of roles in $A$.\\
$P_G(X,Y)$: is the global  joint probability mass function.\\
$P_{r_i}(X,Y)$: is the joint probability mass function  for role $r_i$.
\end{definition}
Note, $f(A)$ is $D(P_A(X,Y) \parallel P_G(X,Y)) $ as per Definition \ref{def:SPRAP}. 

\begin{definition}
For the cost function associated with $RISK_{MI}$ as per definition of Equation \ref{eq:cost}, we define the measure of disclosure  $g_i^A$ as following: \\
\begin{eqnarray*}
g_i^A &= &| MI_A(X,Y) -MI_G(X,Y)|\\
&   - & | MI_{r_i}(X,Y) -MI_G(X,Y)|  |
\end{eqnarray*}
Where:\\
$MI_A(X,Y)$: is the mutual information between random variables. $X$ and  $Y$ calculated based on data accessed by the  set of roles in $A$.\\
$MI_G(X,Y)$: is the global mutual information between  $X$ and  $Y$.\\
$MI_{r_I}$: is the mutual information between  $X$ and $Y$ for role $r_i$.
\end{definition}
Note, $f(A)$ is $MI_A(X,Y) $ as per Definition \ref{def:SPRAP}. 

For an RBAC policy we define the \textit{Property Attackability} ($PA$) parameter as a measure corresponding to the maximum  risk associated with disclosure of the global property/knowledge for a given policy. It is given as $PA = \sum_{r_i \in R} f(r_i)  $. Accordingly, we can define the \emph{quality of risk reduction} $(\Delta)$ as  the second metric which describes the  relative difference between  $PA$  and the risk $RISK_{Div}$ and $RISK_{MI}$ associated  with the properties $Div$ and $MI$, respectively. 

Formally,
\begin{equation}
\label{eq:QoR}
\Delta_{Div} = \frac{(PA - RISK_{Div})}{PA}
\end{equation}
\begin{equation}
\label{eq:QoR}
\Delta_{MI} = \frac{(PA - RISK_{MI})}{PA} 
\end{equation}

Note, $ 1 \le \Delta \le 0$.

We define the  third metric know as  \textit{Discriminator Index} ($DI$)  which is concerned with the performance of heuristics at the role level.  In particular, $DI$  is an indirect indicator of performance of heuristic in term of risk reduction per role. Semantically, $DI$ provides  information about the  quality of reduction provided by a heuristic at  the role level, and indicates disproportionality in terms of risk management over all roles. Formally, it is defined as following: 
\begin{definition}
Given a scheduling heuristic, DI for a heuristic can be formally defined by extending the definition of generic discriminator index in \cite{jain1984quantitative}. For this purpose, given a role  $r_i$, we define the property attackability ($PA_i $), the associated risk ($RISK(r_i) $), and the role quality of risk reduction $\Delta_i$ as follows:\\
\begin{eqnarray*}
PA_i &=& f(r_i)\\
\Delta_i &= &(PA_i - RISK(r_i))  
\end{eqnarray*}
Accordingly, DI is defined as 
\begin{equation}
\label{eq:DI}
 DI = 1- \frac{(\sum_{i=1}^n \Delta_i)^2}{n\times \sum_{i=1}^{n}(\Delta_i)^2} 
\end{equation}
\end{definition}



